Talos: Neutralizing Vulnerabilities with Security Workarounds for Rapid Response

Considerable delays often exist between the discovery of a vulnerability and the issue of a patch. One way to mitigate this window of vulnerability is to use a configuration workaround, which prevents the vulnerable code from being executed at the cost of some lost functionality -- but only if one is available. Since program configurations are not specifically designed to mitigate software vulnerabilities, we find that they only cover 25.2% of vulnerabilities. To minimize patch delay vulnerabilities and address the limitations of configuration workarounds, we propose Security Workarounds for Rapid Response (SWRRs), which are designed to neutralize security vulnerabilities in a timely, secure, and unobtrusive manner. Similar to configuration workarounds, SWRRs neutralize vulnerabilities by preventing vulnerable code from being executed at the cost of some lost functionality. However, the key difference is that SWRRs use existing error-handling code within programs, which enables them to be mechanically inserted with minimal knowledge of the program and minimal developer effort. This allows SWRRs to achieve high coverage while still being fast and easy to deploy. We have designed and implemented Talos, a system that mechanically instruments SWRRs into a given program, and evaluate it on five popular Linux server programs. We run exploits against 11 real-world software vulnerabilities and show that SWRRs neutralize the vulnerabilities in all cases. Quantitative measurements on 320 SWRRs indicate that SWRRs instrumented by Talos can neutralize 75.1% of all potential vulnerabilities and incur a loss of functionality similar to configuration workarounds in 71.3% of those cases. Our overall conclusion is that automatically generated SWRRs can safely mitigate 2.1x more vulnerabilities, while only incurring a loss of functionality comparable to that of traditional configuration workarounds.

==> abstract.tex <==
Configuration workarounds offer an alternative to neutralizing disclosed vulnerabilities when there is no patch available or when it is not possible to apply a patch.  However, configuration settings were never designed to neutralize vulnerabilities and thus offer limited coverage and precision when it comes to this task.

In this work, we propose a dedicated vulnerability workaround mechanism called a {\em Field Programmable Security Workaround} (SWRR), which offers the same benefits of configuration workarounds, but with improved coverage and precision over existing configuration workarounds.  To evaluate the idea of SWRRs, we implement Talos, a compiler tool can automatically instrument application source code with SWRRs.  We evaluate Talos-instrumented SWRRs on... 

==> coverage.tex <==
%To evaluate coverage, we measure the percentage of functions covered by SWRRs in four applications, which is shown in the Talos column in Table~\ref{tbl:coverage}.  We compare this with the Coverage column in Table~\ref{tbl:study}, which gives the percentage of functions covered by existing configuration options, i.e. functions have workarounds.  

From our evaluation, we found that the set of functions covered by Talos and the set of functions covered by configuration options sometimes are quite different. Hence we are interested in two numbers: the percentage of functions that SWRR can cover but do not have workarounds, which shows the benefits of Talos, and the percentage of functions that SWRR cannot cover but have workarounds, which shows the limitations of Talos. We measured the two numbers for four applications, and put the results in the "Talos - Work." column and the "Work. - Talos" column in Table~\ref{tbl:coverage}, respectively. Finally we computed the percentage of functions that can be covered when SWRR and configuration workarounds are both leveraged and show the result in the "Overall" column.

\begin{table}
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{App.} & \textbf{Overall} & \textbf{Talos - Work.} & \textbf{Work. - Talos} \\
\hline
lighttpd & 100\% & 74\% & 0\% \\
\hline
apache & 82\% & 8\% & 50\% \\
\hline
squid & 46\% & 3\% & 38\% \\
\hline
proftpd & 66\% & 30\% & 13\% \\
\hline
\end{tabular}
\caption{Coverage of SWRR.}
\label{tbl:coverage}
\end{table}

As we can see, Talos outperforms workarounds for lighttpd and proftpd, which are the two applications that have the lowest coverage of workarounds as shown in Table~\ref{tbl:error}. 

